Remember This Event That Year? Assessing Temporal Information and Reasoning in Large Language Models

Large Language Models (LLMs) are increasingly ubiquitous, yet their ability to retain and reason about temporal information remains limited, hindering their application in real-world scenarios where understanding the sequential nature of events is crucial. Our study experiments with 12 state-of-the-art models (ranging from 2B to 70B+ parameters) on a novel numerical-temporal dataset, \textbf{TempUN}, spanning from 10,000 BCE to 2100 CE, to uncover significant temporal retention and comprehension limitations. We propose six metrics to assess three learning paradigms to enhance temporal knowledge acquisition. Our findings reveal that open-source models exhibit knowledge gaps more frequently, suggesting a trade-off between limited knowledge and incorrect responses. Additionally, various fine-tuning approaches significantly improved performance, reducing incorrect outputs and impacting the identification of 'information not available' in the generations. The associated dataset and code are available at (https://github.com/lingoiitgn/TempUN).

==> notused.tex <==
% Tables individual
% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccccccccc}  \hline
% \multicolumn{1}{l}{\textbf{}} & \multicolumn{3}{c}{\texttt{mistral-instruct}} & \multicolumn{3}{c}{\texttt{phi-2}} & \multicolumn{3}{c}{\texttt{llama-2-chat}} \\ \hline
% \multicolumn{1}{l}{\textbf{}} &
%   \multicolumn{1}{l}{\textbf{Correct}} &
%   \multicolumn{1}{l}{\textbf{Incorrect}} &
%   \multicolumn{1}{l}{\textbf{NA}} &
%   \multicolumn{1}{l}{\textbf{Correct}} &
%   \multicolumn{1}{l}{\textbf{Incorrect}} &
%   \multicolumn{1}{l}{\textbf{NA}} &
%   \multicolumn{1}{l}{\textbf{Correct}} &
%   \multicolumn{1}{l}{\textbf{Incorrect}} &
%   \multicolumn{1}{l}{\textbf{NA}} \\  \hline
% $DB$                            & \textbf{37.21}   & \textbf{51.22}   & \textbf{11.57}   & 10.9    & 89.1    & 0     & 20.86   & 76.17  & 2.97  \\
% $RB$                            & \textbf{42.92}   & 57.08   & 0       & 0       & 96.99   & \textbf{3.01}  & 44.87   & \textbf{55.13}  & 0     \\
% $WB$                            & 19.76   & 80.24   & 0       & 18.19   & 81.81   & 0     & \textbf{21.63}   & \textbf{78.37}  & 0     \\
% $MMB$                           & \textbf{23.12}   & \textbf{63.53}   & \textbf{13.35}   & 7.69    & 92.16   & 0.15  & 14.89   & 81.1   & 4.01  \\
% $RAB$                           & \textbf{33.62}   & \textbf{66.38}   & 0       & 9.34    & 88.54   & \textbf{2.11}  & 21.5    & 78.5   & 0     \\
% $TB$                            & \textbf{7.73}    &\textbf{ 70.71}   & \textbf{21.56}   & 5.79    & 93.04   & 1.17  & 4.88    & 92.75  & 2.38  \\  \hline
% \end{tabular}%
% }
% \caption{\label{table:num-metrics_results}
% The performance assessment of different models with the MCQ-based evaluation strategies for each category. Here, `Correct', `Incorrect', and `NA' represents the percentage of correct generations, incorrect generations, and LLMs generation of information not available, respectively.}
% \end{table*}

% \begin{table*}[]
% \centering
% \begin{tabular}{ccccccc}
% \hline
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{\texttt{gemini-pro}} & \multicolumn{3}{c}{\texttt{gpt-4}} \\ \hline
% \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{\textbf{Correct}} &
%   \multicolumn{1}{l}{\textbf{Incorrect}} &
%   \multicolumn{1}{l}{\textbf{NA}} &
%   \multicolumn{1}{l}{\textbf{Correct}} &
%   \multicolumn{1}{l}{\textbf{Incorrect}} &
%   \multicolumn{1}{l}{\textbf{NA}} \\ \hline
% $DB$                 & 0        & 0        & 0        & 0       & 0      & 0      \\
% $RB$                 & 0        & 0        & 0        & 0       & 0      & 0      \\
% $WB$                 & 0        & 0        & 0        & 0       & 0      & 0      \\
% $MMB$                & 0        & 0        & 0        & 0       & 0      & 0      \\
% $RAB$                & 0        & 0        & 0        & 0       & 0      & 0      \\
% $TB$                 & 0        & 0        & 0        & 0       & 0      & 0      \\ \hline
% \end{tabular}
% \caption{\label{table:num-metrics_results}
% The performance assessment of different models with the MCQ-based evaluation strategies for each category. Here, `Correct', `Incorrect', and `NA' represents the percentage of correct generations, incorrect generations, and LLMs generation of information not available, respectively. \textcolor{blue}{FILL VALUES!}} 
% \end{table*}



% \begin{table*}[]
% \centering
% \begin{tabular}{lp{0.9cm}lllllllll} \hline
% \textbf{Model}            & \textbf{Metrics} & \multicolumn{1}{l}{\textbf{C$1$}} & \multicolumn{1}{l}{\textbf{C$2$}} & \multicolumn{1}{l}{\textbf{C$3$}} & \multicolumn{1}{l}{\textbf{C$4$}} & \multicolumn{1}{l}{\textbf{C$5$}} & \multicolumn{1}{l}{\textbf{C$6$}} & \multicolumn{1}{l}{\textbf{C$7$}} & \multicolumn{1}{l}{\textbf{C$8$}} & \multicolumn{1}{l}{\textbf{All}} \\ \hline
% \texttt{mistral-instruct} & $DB$             & 40.7                              & 23.25                             & 41.39                             & 28.85                             & 30.45                             & 36.83                             & 45.86                             & 31.22                             & \textbf{37.21}                            \\
%                           & $RB$             & 19.39                             & 13.03                             & 17.98                             & 20.58                             & 31.43                             & 28.9                              & 26.2                              & 29.62                             & \textbf{23.12 }                           \\
%                           & $WB$             & 23.57                             & 30.42                             & 37.12                             & 19.01                             & 36.12                             & 34.27                             & 43.24                             & 44.06                             & \textbf{33.62}                            \\
%                           & $RAB$            & 22.83                             & 9.54                              & 1.91                              & 7.54                              & 8.13                              & 5.1                               & 2.76                              & 3.35                              &\textbf{ 7.73 }                            \\
%                           & $MMB$            & 47.25                             & 52.24                             & 15.82                             & 61                                & 28.53                             & 65.49                             & 13.76                             & 70.13                             & 42.92                            \\
%                           & $TB$             & 6.84                              & 10.74                             & 25.49                             & 18.11                             & 19.72                             & 36.35                             & 22.16                             & 16.37                             & 19.76                            \\ \hline
% \texttt{llama-2-chat}     & $DB$             & 7.25                              & 12.47                             & 9.9                               & 4.8                               & 15.54                             & 11.27                             & 13.68                             & 10.96                             & 10.9                             \\
%                           & $RB$             & 4.14                              & 6.09                              & 2.3                               & 8.41                              & 12.43                             & 5.44                              & 13.39                             & 12.39                             & 7.69                             \\
%                           & $WB$             & 10.7                              & 8.5                               & 1.28                              & 6.53                              & 11.88                             & 8.08                              & 17.89                             & 13.42                             & 9.34                             \\
%                           & $RAB$            & 1.11                              & 2.89                              & 11.21                             & 6.07                              & 11.96                             & 5.24                              & 2.02                              & 3.81                              & 5.79                             \\
%                           & $MMB$            & 0                                 & 0                                 & 0                                 & 0                                 & 0                                 & 0                                 & 0                                 & 0                                 & 0                                \\
%                           & $TB$             & 19.39                             & 19.32                             & 12.53                             & 17.92                             & 18.27                             & 14.56                             & 22.83                             & 23.88                             & 18.19                            \\ \hline
% \texttt{Phi-2}            & $DB$             & 27.04                             & 14.9                              & 18.97                             & 19.73                             & 22.21                             & 19.23                             & 25.18                             & 18.82                             & 20.86                            \\
%                           & $RB$             & 10.16                             & 8.3                               & 14.05                             & 12.82                             & 20.43                             & 19.76                             & 17.49                             & 17.06                             & 14.89                            \\
%                           & $WB$             & 19.1                              & 13.91                             & 17.82                             & 25.69                             & 21.29                             & 24.32                             & 31.66                             & 21.77                             & 21.5                             \\
%                           & $RAB$            & 2.17                              & 0.64                              & 4.16                              & 4                                 & 9.02                              & 8.28                              & 5.46                              & 5.34                              & 4.88                             \\
%                           & $MMB$            & 47.09                             & 52.54                             & 12.76                             & 68.06                             & 63.69                             & 13.72                             & 40.43                             & 69.52                             & \textbf{44.87}                            \\
%                           & $TB$             & 23.81                             & 16.31                             & 24.2                              & 24.17                             & 15.65                             & 23.2                              & 23.45                             & 23.88                             & \textbf{21.63}                            \\ \hline
% \end{tabular}
% \caption{\label{table:num-metrics}
% The performance assessment of different models with the MCQ-based evaluation strategies for each category. Here, 'All' represents the combined values for all the categories. }
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{lp{9cm}p{5cm}} \hline
% \textbf{Metric} &
%   \textbf{Example} &
%   \textbf{Explaination} \\  \hline
% $EM$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 43,846.47 USD\end{tabular} &
%   If the truth is exaclty equal to the prediction for all n inputs. \\ \hline
% $AE$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}AEi = Truth - Prediction\\ Average for all n inputs.\end{tabular} \\ \hline
% $OE$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%   OE = AE1 + AE2 + .. + AEi \\ \hline
% $RS$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%   The oldest year a model can remember. \\ \hline
% $DCI$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%    \\ \hline
% $IvF$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%    \\ \hline
% $PC$ &
%   \begin{tabular}[c]{@{}l@{}}Prompt: In 2011, the GDP of France was?\\ Truth: 43,846.47 USD, Prediction: 42,231.45 USD\end{tabular} &
%    \\  \hline
% \end{tabular}
% \caption{\label{tab:metricsexam}Definitions of metrics using examples. \textcolor{blue}{UPPDATING THIS TABLE!}}
% \end{table*}
% \subsection{Numerical-based Evaluation Strategy}
% \label{sec:metric}
% We define the evaluation strategy for the numerical-based generations in this section. We define the notations used in the metrics in Table~\ref{tab:notations}. The metrics used to assess the models for numerical and non-numerical facts are as follows:


% \begin{table}
% \centering
% \begin{tabular}{ll}
% \hline
% \textbf{Notations}               & \textbf{Definition}  \\ \hline
% $x$              & Simple Prompt  \\ 
% $y$ & Year \\
% $o$ & Generation from Model \\ 
% $t$ & At specific time-stamp \\
% $N$ & Number of instances 
% \\ \hline
% \end{tabular}
% \caption{\label{tab:notations}Notations used in the metrics. \textcolor{blue}{UPPDATING THIS TABLE!}}

% \end{table}


% \subsubsection{Exact Match ($EM$)}
% $EM$ is derived when the prediction differs from the ground truth. Let $o$ be the ground truth, and $o'$ is the prediction for the $i$-th year $y_{i}$. Mathematically, for the entire test set ($T$) where $N = |T|$, we define $EM$ as,
%     \begin{equation}
%     EM_{avg} = \frac{\sum_{t\: \epsilon\: T; \: (y^{t'}_{i},o^{t'})=(y^{t}_{i},o^{t})}^{} 1}{N}
%     \end{equation}


% \subsubsection{Normalised Absolute Error ($AE$)}
% Absolute error is robust to outliers metric \citep{mae}, but the scale of numbers predicted by the LMs is different. Hence, we normalize the predicted number by $10^{n-1}$ where $n$ is the number of digits before the decimal place in the given number. Hence, the predicted number will be in the range of $(-10, 10)$. For entire test dataset the Mean Normalised AE is defined as,
%     \begin{equation}
%     AE_{avg} = \frac{\sum_{t\: \epsilon\: T;}|\frac{o_{t}' - o_{t}}{10^{n-1}}|}{N}
%     \end{equation}
%     where $n$ is the number of digits in the integer part of any real number is defined as,
%     \begin{equation}
%         n = \lfloor log_{10}(|o_{t}'-o_{t}|)+1 \rfloor
%     \end{equation}

% \subsubsection{Exact Ordering ($O_{E}$)} 
% $O_{E}$ is defined as the sum of $AE$ for each number in the prediction sequence for every instance in the test set.

% \subsubsection{Remeberance Score ($RS$)}
% $RS$ for a model is the largest year span, with the $EM$ being above or equal to a threshold (Ideally, the threshold is one). 

% \subsubsection{Digit Count Impact Score ($DCI$)}
% $DCI$ aims to examine the model's ability to handle numbers based on the number of digits in the number. After categorizing the output based on the length of the number, $DCI$ represents the maximum length for which the $AE$ is the least.

% \subsubsection{Integer vs. Float Score ($IvF$)}
% $IvF$ for a test dataset is defined as the average number of times the model correctly predicts integer or floating point number

% \subsubsection{Polarity Correctness ($PC$)}
% $PC$ examines the model's ability to correctly identify the number's polarity (negative and positive numbers). Mathematically defined as
%     \begin{equation}
%         PC = \frac{\sum_{t\: \epsilon\: T; \: (o^{t'} \times\: o^{t}) \geq 0}^{} 1}{N}
%     \end{equation} 

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{lp{10cm}p{5cm}} \hline
% \textbf{Metric} &
%   \textbf{Example} &
%   \textbf{Explaination} \\ \hline
% \textit{Exact Match} ($EM$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 2011, the GDP of France was?}}\\ \textbf{Truth}: \textcolor{green}{43,846.47 USD}, \textbf{Prediction}: \textcolor{blue}{43,846.47 USD}\end{tabular} &
%   \textit{If the truth is exactly equal to the prediction for all n inputs.} \\ \hline
% \textit{Normalized Absolute Error} ($AE$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 2011, the GDP of France was?}}\\ \textbf{Truth}: \textcolor{green}{43,846.47 USD}, \textbf{Prediction}: \textcolor{blue}{42,231.45 USD}\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}
%   \textit{$AE_i$ = Truth - Prediction;}\\ \textit{Average for all n inputs.}\end{tabular} \\ \hline
% \textit{Exact Ordering }($OE$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{What was the GDP of France from 2015 to 2017?}}\\ \textbf{Truth}: \textcolor{green}{36,652.92 USD, 37,062.53 USD, 38,781.05 USD}, \\ \textbf{Prediction}: \textcolor{blue}{42,231.45 USD, 47,062.53 USD, 48,154.51 USD}\end{tabular} &
%   $OE$ = $AE_1$ + $AE_2$ + .. + $AE_i$ \\ \hline
% \textit{Remembrance Score} ($RS$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 1974, the GDP of France was?}}\\ \textbf{Truth}: \textcolor{green}{43,846.47 USD}, \textbf{Prediction}: \textcolor{blue}{42,231.45 USD}\end{tabular} &
%   \textit{The oldest year for which a model can remember.} \\ \hline
% \textit{Digit Count Impact Score} ($DCI$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 2011, the GDP of France was?}}\\ \textbf{Truth}: \textcolor{green}{43,846.47 USD}, \textbf{Prediction}: \textcolor{blue}{42,231.45 USD}\end{tabular} &
%   \textit{The maximum length (Number of digits) for which the AE is least.} \\ \hline
% \textit{Integer vs Float} ($IvF$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 2011, what was the population and GDP of}} \\ \textcolor{darkgray}{\textit{France?}}\\ \textbf{Truth}: \textcolor{green}{65,276,983 and 43,846.47 USD}, \\ \textbf{Prediction}: \textcolor{blue}{65,124,123 and 42,231.45 USD}\end{tabular} &
%   \textit{When the model corrects predicts an integer or float number.} \\ \hline
% \textit{Polarity Correctness} ($PC$) &
%   \begin{tabular}[c]{@{}l@{}}\textbf{Prompt}: \textcolor{darkgray}{\textit{In 2011, what was the stock value of Apple in}}\\ \textcolor{darkgray}{\textit{France?}}\\ \textbf{Truth}: \textcolor{green}{-12.45 USD}, \textbf{Prediction}: \textcolor{blue}{10.23 USD}\end{tabular} &
%   \textit{Does the model capture the number's polarity?}\\ \hline
% \end{tabular}%
% }
% \caption{\label{tab:metricsexam}The numerical-based metrics.}
% \end{table*}
% \begin{table*}[]
% \centering
% \begin{tabular}{lllllllllll} \hline
% \textbf{Model} &
%   \textbf{Metrics} &
%   \textbf{$C1$} &
%   \textbf{$C2$} &
%   \textbf{$C3$} &
%   \textbf{$C4$} &
%   \textbf{$C5$} &
%   \textbf{$C6$} &
%   \textbf{$C7$} &
%   \textbf{$C8$} &
%   \textbf{All} \\ \hline
% \texttt{mistral-instruct}       & $EM$  &  &  &  &  &  &  &  &  &  \\
%               & $AE$  &  &  &  &  &  &  &  &  &  \\
%               & $OE$  &  &  &  &  &  &  &  &  &  \\
%               & $RS$  &  &  &  &  &  &  &  &  &  \\
%               & $DCI$ &  &  &  &  &  &  &  &  &  \\
%               & $IvF$ &  &  &  &  &  &  &  &  &  \\
%               & $PC$  &  &  &  &  &  &  &  &  &  \\ \hline
% \texttt{llama-2-chat}       & $EM$  &  &  &  &  &  &  &  &  &  \\
%               & $AE$  &  &  &  &  &  &  &  &  &  \\
%               & $OE$  &  &  &  &  &  &  &  &  &  \\
%               & $RS$  &  &  &  &  &  &  &  &  &  \\
%               & $DCI$ &  &  &  &  &  &  &  &  &  \\
%               & $IvF$ &  &  &  &  &  &  &  &  &  \\
%               & $PC$  &  &  &  &  &  &  &  &  &  \\ \hline
% \texttt{gpt-3.5-turbo} & $EM$  &  &  &  &  &  &  &  &  &  \\
%               & $AE$  &  &  &  &  &  &  &  &  &  \\
%               & $OE$  &  &  &  &  &  &  &  &  &  \\
%               & $RS$  &  &  &  &  &  &  &  &  &  \\
%               & $DCI$ &  &  &  &  &  &  &  &  &  \\
%               & $IvF$ &  &  &  &  &  &  &  &  &  \\
%               & $PC$  &  &  &  &  &  &  &  &  &  \\ \hline
% \texttt{gpt2-xl}       & $EM$  &  &  &  &  &  &  &  &  &  \\
%               & $AE$  &  &  &  &  &  &  &  &  &  \\
%               & $OE$  &  &  &  &  &  &  &  &  &  \\
%               & $RS$  &  &  &  &  &  &  &  &  &  \\
%               & $DCI$ &  &  &  &  &  &  &  &  &  \\
%               & $IvF$ &  &  &  &  &  &  &  &  &  \\
%               & $PC$  &  &  &  &  &  &  &  &  &  \\ \hline
% \texttt{t5-large}            & $EM$  &  &  &  &  &  &  &  &  &  \\
%               & $AE$  &  &  &  &  &  &  &  &  &  \\
%               & $OE$  &  &  &  &  &  &  &  &  &  \\
%               & $RS$  &  &  &  &  &  &  &  &  &  \\
%               & $DCI$ &  &  &  &  &  &  &  &  &  \\
%               & $IvF$ &  &  &  &  &  &  &  &  &  \\
%               & $PC$  &  &  &  &  &  &  &  &  &  \\ \hline
% \end{tabular}
% \caption{\label{table:mcq-metrics}
% The performance assessment of different models with the numerical-based evaluation strategies for each category.}

% \end{table*}

